Holographic Complexity in dS$_{d+1}$

We study the CV, CA, and CV2.0 approaches to holographic complexity in $(d+1)$-dimensional de Sitter spacetime. We find that holographic complexity and corresponding growth rate presents universal behaviour for all three approaches. In particular, the holographic complexity exhibits `hyperfast' growth [arXiv:2109.14104] and appears to diverge with a universal power law at a (finite) critical time. We introduce a cutoff surface to regulate this divergence, and the subsequent growth of the holographic complexity is linear in time.

==> sections/sectionCold.tex <==
% !TEX root = ../CVdS03.tex
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%


In this section, we study the CA proposal \reef{defineCA} in $\dS_{d+1}$. In particular, we suppose that the complexity is given by the gravitational action evaluated on the WdW patch anchored on the stretched horizon (\eg see figure \ref{fig:WdW}).  Schematically, the complexity is then given by
\begin{equation}\label{eq:CAeq}
\ca= \frac{1}{\pi}\left(I_{\rm{bulk}}  + I_{\mt{GHY}} +  I_{\rm null} +I_{\rm{joint}} + I_{\rm{ct}}  \right)\,,
\end{equation}
Apart from the usual bulk action $I_{\rm{bulk}}$, we have included the appropriate boundary terms (\ie $I_{\mt{GHY}},\, I_{\rm null},\, I_{\rm{ct}}$) for the various codimension-one boundary segments and the joint terms $I_{\rm{joint}}$ for the codimension-two surfaces where the boundary segments intersect \eg \cite{Lehner:2016vdi,Carmi:2016wjl}. \rcm{I would prefer to use the conventions in Appendix A of \cite{Carmi:2016wjl}.} 

The bulk contribution to the complexity is given by the usual Einstein-Hilbert action with positive cosmological constant. Since de Sitter space has constant scalar curvature, the bulk term is simply proportional to the spacetime volume of the WdW patch,
\begin{equation}\label{eq:Ibulk}
    \frac1\pi\,I_{\rm bulk}= \frac{1}{16\pi ^2\GN}\int d^{d+1}x \sqrt{-g}\(R-\frac{d(d-1)}{L^2}\)=\frac{d \, V_{\mt{WdW}} }{8\pi ^2\GN L^2}= \frac{d}{8 \pi^2}\, \cvv \,.
\end{equation}
Since we saw that $\cvv$ diverges as  $\tau\to \tau_{\infty}$ (see~eq.~\eqref{eq:VWdWaround}), this bulk term produces similar divergent behaviour in $\ca$.
Hence we will regulate the results with a cutoff surface at 
$r=\rmax=L/\veps$, just as in the previous section. This term will  play a role for $\tau \gtrsim \tauinf$, when the WdW patch has encountered the regulator surface and has a spacelike boundary at $r=\rmax$.

\subsubsection*{Early time evolution of CA ($\tau \le \tau_{\infty}$)}
%

As discussed in the previous section, at early times $\tau \le \tau_{\infty}$, the WdW patch has four null boundaries designated in eq.~\reef{bound77}.  To evaluate the corresponding boundary and joint terms, we must define the normals for these surfaces. Following the prescription given in appendix A of \cite{Carmi:2016wjl},
we choose \rcm{two boundaries on the right hand side?? introduce notation for all four boundaries.}
\begin{equation}\label{nullvec}
\begin{split}
   k _{\mu}dx^\mu&= \alpha\, du|_{u=u_{\rm max}} =\alpha \(dt-dr/f(r)\)|_{u=u_{\rm max}}\,,\\
k'_{\mu}dx^\mu&= -\alpha'\, dv|_{v=v_{\rm max}} =- \alpha' \(dt+dr/f(r)\)|_{v=v_{\rm max}}\,,
\end{split}
\end{equation}
where $\alpha$ and $\alpha'$ are arbitrary (positive) constants. \rcm{confirm sign} \rcm{****}

\rcm{Two questions: a) Does the counterterm in Appendix B(?) of \cite{Lehner:2016vdi} vanish for affinely parametrized null vectors? b) The overall normalization of these vectors is arbitrary, \eg I could replace $k\to \alpha k$. Does $\alpha$ cancel in the full action when we add in the two joint terms at either end of the corresponding null surface? }  \eiv{a) Yes, the counter term vanishes. Do you think it would be a good idea to discuss this in more detail in the text? \rcm{Are you sure the counterterm doesn't kill the $\alpha$'s?} b) They should not drop out in general, I will update the text to make this explicit. } 

we choose $k$ and $k'$ to be affinely parametrized. 

\rcm{***} Below, we choose the null boundary segments to be affinely parametrized, which sets the corresponding boundary terms to zero. 

The joint terms take the form
\begin{equation}
    I_{\rm joint}=\frac{1}{8\pi \GN}\int_{\text{joint}}\log \(   {\frac{|k\cdot k'|}{2}}  \)dS,
\end{equation}
where $k$ and $k'$ are future-oriented normals to the two intersecting null segments.
For the uppermost joint of the WdW patch, it is straightforward to get \smr{changes $r$ to $r_+(\tau)$}
\rcm{Seems Eivind intended this formula for all four corners.}
\begin{equation}
   k\cdot k'=\frac{2\alpha\alpha'}{f\(r_+\)}   \,,  
   %=-\alpha\alpha'\frac{(1-UV)^2}{2UV},
\end{equation}

\rcm{write out result of all boundary terms}


As we approach the critical time $\tau \to \tauinf$, the radius of upper joint defined in eq.~\eqref{eq:rpm} is divergent in terms of 
\begin{equation}
 \lim_{\tau\to \tau_{\infty}}  \frac{r_+ (\tau)}{L} \approx  \frac{1}{\tauinf -\tau} +\frac{1}{3} (\tauinf -\tau ) + \mathcal{O}\(  (\tauinf -\tau )^2 \) \,,
\end{equation}
which gives a divergent contribution to holographic complexity $\ca$. The other joint terms will not play a significant role in the following discussion. \smr{Added one more series expansion.}

Similarly to the case for the CV2.0 proposal, $\ca$ diverges as the boundary time approaches $\tau_{\infty}$. However, in this case there are divergent contributions coming both from the spacetime volume of the WdW patch (or the bulk action) and the joint terms. Indeed, we have  \smr{The following result is valid for $d>1$. For $d=1$, the logarithmic term from $\cvv$ also contributes to the leading term. }

\begin{equation}
\lim_{\tau\to \tau_{\infty}}\ca \approx \frac{N}{\pi^2}\left(\frac{1}{(d-1)(\tau_{\infty}-\tau)^{d-1}} - \frac{2\log\left(\frac{\tau_{\infty}-\tau}{\alpha\alpha'}\right)}{(\tau_{\infty}-\tau)^{d-1}}+\mathcal{O}\left(\frac{\log(\tau_{\infty}-\tau)}{(\tau_{\infty}-\tau)^{d-2}}\right)\right) ,
\end{equation}
\rcm{Since this is already an approximation and we are interested in $\tau\to\tauinf$, please, express this in terms of powers of $\tauinf-\tau$ rather than exponentials. Please also remind the reader what the leading divergence in $V_{\mt{WdW}}$ is -- and refer back to the appropriate equation in the previous section.}\eiv{Updated the equation and rewrote some surrounding text}s\smr{Please check the coefficient for the second term.  Is it $\frac{1}{(\tauinf -\tau)^{d-1}}$ without a factor $2$? } 
where non-logarithmic part of the leading order term comes from the bulk action (cf. eqs~\eqref{eq:Ibulk} and~\eqref{eq:VWdWaround}) and the logarithmic part comes from the joint term. \smr{The prefactor of the leading term is given by $\frac{1}{(d-1)} + \log (\alpha \alpha')$. So $\ca$ could be negative if $\alpha \alpha' <<1$? }


\smr{Added the following equation, for the discussion after eq.~\eqref{eq:CAderivativelate}.} 

Similar to CV2.0, we obtain the hyperfast growth for holographic complexity $\ca$ by approaching the critical time $\tauinf$, \viz 
\begin{equation} \label{eq:CAderivativeearly}
\lim_{\tau\to \tau_{\infty}} \frac{d \ca  (\tau \le \tauinf )}{d \tau}\approx \frac{N}{\pi^2} \frac{2}{(\tauinf -\tau)^d}   ++\mathcal{O}\left(\frac{\log(\tau_{\infty}-\tau)}{(\tau_{\infty}-\tau)^{d-2}} \right) \,.
\end{equation}
\smr{We can add a complete expression   $\frac{d \ca  (\tau \le \tauinf )}{d \tau}$ for any early times $\tau \le \tauinf$.}


\subsection{Gravitational action with cutoff}
\begin{figure}[h!]
	\centering
	\includegraphics[width=3.5in]{CaFigfinal.pdf}
	\caption{The complexity evaluated on the WdW patch plotted against the boundary time. The divergent behaviour at $\tau_{\infty}$ is tamed by the introduction of a cutoff surface, which subsequently leads to linear growth at late times. Unlike the case for the spacetime volume, there is a discontinuous jump in the first derivative of the complexity when the WdW patch hits the cutoff surface. Here $L=1$, $\epsilon=0.1$, $\alpha=\alpha'=1$, $d=3$ and $\rho=0.9$. \smr{Could we set $N=1$ to be consistent with other plots?} }
	\label{fig:Cafig}
\end{figure} 	

\smr{Should add the definition of $\ca$ for late times since the definition in eq.~\eqref{eq:CAeq} does not include the contributions from the cut-off surface.
	\begin{equation}
		\begin{aligned}
			I &= I_{\rm{bulk}}  + I_{\mt{GHY}} + I_{\rm{joint}} + I_{\rm null} + I_{\rm{ct}}  \\
			&=  \frac1{16\pi\GN} \int d^{d+1}x \sqrt{-g} \(  {\cal R}+\frac{d(d-1)}{L^2} \)+ \frac{1}{8\pi \GN} \int_{\mt{cut-off}}\!\!\!\!\!   d^{d}x\,\sqrt{|h|}\,K  \\
			&\, + \frac{1}{8\pi \GN} \int_{\rm joints}\!\!\!\!\!  d^{d-2}x\,\sqrt{\sigma}\,a + \frac{1}{8\pi \GN} \int_{\del{\rm WDW}}\!\!\!\!\!  ds\,d^{d-2}\Omega\,\sqrt{\gamma}\,\kappa  + \frac{1}{8\pi \GN} \int_{\del{\rm WDW}}\!\!\!\!\! ds \,d^{d-2}\Omega\,\sqrt{\gamma}\, \Theta \log (\ell_{\rm ct} \Theta) 
			\,. 
		\end{aligned}
		\label{eq:defineCA}
	\end{equation}
}


To tame the divergence we can once again introduce a cutoff surface at $r=\rmax=L/\epsilon$. The cutoff surface gives rise to additional boundary terms in the action. Firstly, we get two joint terms where null segments of the WdW patch intersect the cutoff surface, which take the form
\begin{equation}
    I_{\rm joint}=
    \frac{1}{8\pi \GN}\int_{\rm{joint}}\log{|k\cdot n|} dS,
\end{equation}
where $n$ is a future directed normal vector to the cutoff surface. We will not focus on the joint terms here since $d(k\cdot n)/dt_R=0$, so they only give a constant contribution to the complexity.  More importantly, there will be the usual Gibbons-Hawking term where the extrinsic curvature is integrated over the cutoff surface
\begin{equation}
    I_{\rm cutoff}=\frac{1}{8\pi \GN} \int_{\rm cutoff} K d\Sigma,
\end{equation}
where $K=\nabla_{\mu}n^{\mu}$ is the extrinsic curvature. One can show that the extrinsic curvature is constant on any surface of constant $UV$ (and hence constant $r$) and takes the form
\begin{equation}
    K=-\frac{1+2(2d-1)UV+(UV)^2}{2(1+UV)\sqrt{UV}}.
\end{equation}
It is then a simple matter to integrate $K$ over the cutoff surface, giving a contribution to the complexity of the form
\begin{equation}
     I_{\rm cutoff}\approx-\frac{N}{2\pi }\frac{d}{\epsilon^d}\left[\log U\right]_{U_1}^{U_2},
\end{equation}
where $U_1$ and $U_2$ are coordinates for the two null-spacelike joints on the cutoff surface. At late boundary times the action grows linearly, with the dominant contributions coming from the spacelike Gibbons-Hawking term and the bulk term. Indeed, for $\tau \ge \tau_\ast$  \smr{Changed $\tau>\tauinf $  to $\tau \ge \tau_\ast$ or $\tau \gtrsim \tauinf$} we have 
\begin{equation} \label{eq:CAderivativelate}
    \frac{d \ca  (\tau \ge \tau_{\ast} )}{d \tau}\approx \frac{N}{\pi^2}\frac{(d+
    1)}{\veps^d}+\mathcal{O}\left(\frac{1}{\veps^{d-2}}\right).
\end{equation}
\rcm{Note the replacement $\epsilon\to\veps$. Was that correct?}
As we have seen in section~\ref{sec:CV20}, the evolution of $\cvv$ is continuous in the first derivative when we reach the cutoff surface. For $\ca$ however, both the divergent behaviour as we approach $\tau_{\infty}$ and the subsequent linear growth is altered by the presence of joint and boundary terms. As a result there is a discontinuous jump in the first derivative of $\ca$ when the WdW first intersects the cutoff surface, see Fig.~\ref{fig:Cafig}. Note that the jump has nothing to do with the choice of normalization constants for the null normals, as they affect only the sub-leading (i.e. non-logarithmic in $\tau$) divergent terms for $\tau<\tauinf$ and do not affect the subsequent linear growth. 




%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%



